Diversity-guided Search Exploration for Self-driving Cars Test Generation through Frenet Space Encoding

The rise of self-driving cars (SDCs) presents important safety challenges to address in dynamic environments. While field testing is essential, current methods lack diversity in assessing critical SDC scenarios. Prior research introduced simulation-based testing for SDCs, with Frenetic, a test generation approach based on Frenet space encoding, achieving a relatively high percentage of valid tests (approximately 50%) characterized by naturally smooth curves. The "minimal out-of-bound distance" is often taken as a fitness function, which we argue to be a sub-optimal metric. Instead, we show that the likelihood of leading to an out-of-bound condition can be learned by the deep-learning vanilla transformer model. We combine this "inherently learned metric" with a genetic algorithm, which has been shown to produce a high diversity of tests. To validate our approach, we conducted a large-scale empirical evaluation on a dataset comprising over 1,174 simulated test cases created to challenge the SDCs behavior. Our investigation revealed that our approach demonstrates a substantial reduction in generating non-valid test cases, increased diversity, and high accuracy in identifying safety violations during SDC test execution.

==> frenet-frame.tex <==
\begin{tikzpicture}

%\filldraw[color=red!60, fill=red!5, very thick](-1,0) circle (1.5);
%\fill[blue!50] (2.5,0) ellipse (1.5 and 0.5);
\filldraw[color=red!60, fill=red!5, very thick] (0,0.5) circle (0.1);
\draw[thick] (-2,2) .. controls (0,0) .. (2,2);
\draw[->] (0,0.5) -- (1,0.5);
\draw[->] (0,0.5) -- (0,1.5);
\node[] at (0.3,1.5) {$N$};
\node[] at (1.2,.5) {$T$};

\end{tikzpicture}
